API Is Enough: Conformal Prediction for Large Language Models Without Logit-Access

This study aims to address the pervasive challenge of quantifying uncertainty in large language models (LLMs) without logit-access. Conformal Prediction (CP), known for its model-agnostic and distribution-free features, is a desired approach for various LLMs and data distributions. However, existing CP methods for LLMs typically assume access to the logits, which are unavailable for some API-only LLMs. In addition, logits are known to be miscalibrated, potentially leading to degraded CP performance. To tackle these challenges, we introduce a novel CP method that (1) is tailored for API-only LLMs without logit-access; (2) minimizes the size of prediction sets; and (3) ensures a statistical guarantee of the user-defined coverage. The core idea of this approach is to formulate nonconformity measures using both coarse-grained (i.e., sample frequency) and fine-grained uncertainty notions (e.g., semantic similarity). Experimental results on both close-ended and open-ended Question Answering tasks show our approach can mostly outperform the logit-based CP baselines.

==> Sections/ethics.tex <==
\section*{Ethics Statement}
% Scientific work published at ACL 2023 must comply with the ACL Ethics Policy.\footnote{\url{https://www.aclweb.org/portal/content/acl-code-ethics}} We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).
This paper does not raise any ethical concerns. The data and resources we use are all open-sourced and openly accessible. Access to Llama-2 is available upon request with permission from Meta.

==> Sections/methodology_old.tex <==
\section{Methodology}
\label{motivation}

Given the context of black-box LLMs, a question arises: \textit{Can we employ conformal prediction without white-box access to LLMs, i.e. without requiring access to token logits or other detailed information about the model's structure?} Initially, we proposed approximating real probabilities through a sufficiently large number of samples. This allows us to leverage frequency to confidently substitute for probabilities. However, our theoretical analysis indicates that a minimum of 9604 samples is required to achieve 95\% confidence results with a 1\% margin of error, as supported by Lemma \ref{lemma31}. Therefore, the implementation is impractical due to computational constraints.
%\subsection{Minimum Sample Size for Confident Probability Estimation}
\begin{lemma}[Minimum Sample Size for Confident Probability Estimation]
\label{lemma31}
Let $freq(y)$ denote the frequency of outcome $y$ in the sampling, $N_{\text{total}}$ represent the total number of samplings, $p_i$ be the desired estimated probability, $\epsilon$ be the estimation error, and $\alpha$ be the target confidence level. To determine the minimum sample size for confident probability estimation, for any given $\epsilon > 0$ and $0 < \alpha < 1$, the following inequality must hold:
\begin{equation}
   P\left\{\left|\frac{freq(y)}{N_{\text{total}}} - p_i\right| \leq \epsilon\right\} \geq \alpha 
\end{equation}
Then, the minimum sample size $N_{total}$ satisfying this inequality is given by:
\begin{equation}
    N_{total} \geq \left(\frac{u_{\alpha}}{2\epsilon}\right)^2
\end{equation}
where $u_{\alpha}$ is the quantile of the standard normal distribution corresponding to the confidence level $\alpha$. The proof is given in Appendix \ref{sec:appendix}.
\end{lemma}

\subsection{Coarse-grained Nonconfority Measure}
Then, inspired by the principles of nonconformity measures \cite{shafer2008tutorial}, while existing works employ logits or hidden activations for nonconformity measures, the primary focus lies in the rankings of uncertainty inherent in logits or hidden activations rather than the values themselves. Therefore, as long as we can establish rankings of the model's uncertainty (nonconformity), effective conformal prediction is feasible. Further, self-consistency theory gives that a repetitively sampled response is viewed as a form of consistency linked to higher confidence in the response. To empirically validate this intuition, we randomly select 2000 questions from the TriviaQA dataset \cite{joshi2017triviaqa}. Then we conduct 20 samplings using LLaMA-7b \cite{touvron2023llama} and retrieve the logits, subsequently calculating real probabilities. The empirical findings are shown in Figure \ref{FIG:1a}. We observe that as the response frequency increases, the average real probability rises proportionally, indicating a greater level of certainty and confidence in the response.


However, only considering frequency, a coarse-grained uncertainty notion, leads to a concentration issue of scores, resulting in scores that do not reflect nonconformity differences between responses with the same frequency within each prompt and between different prompts. For example, in Figure \ref{FIG:overview}, it contains the concentration issue with responses of different prompts (e.g., "\textit{Big Bill Broonzy}" and "\textit{Joan Rivers}") and responses within a prompt (e.g., "\textit{Bill Boonzy}" and "\textit{Sir William Rockington}").

To resolve the concentration issue, inspired by self-consistency theory \cite{wang2022self, li2022advance}, we firstly incorporate normalized entropy, a prompt-wise fine-grained uncertainty notion, to mitigate the concentration issue in different prompts. The normalized entropy is a measure of the uncertainty or diversity in the model's predictions when generating responses to a given prompt, which is computed as (\ref{ne_Eq}). Empirically, Figure \ref{FIG:1b} demonstrates that as normalized entropy increases, the number of unanswered questions also increases, indicating a rise in uncertainty. Besides, aiming to mitigate concentration issues within a prompt, we incorporate semantic similarity, a response-wise fine-grained uncertainty notion, to measure the likeness between each non-Top-1 response and the Top-1 response within a prompt.
\begin{equation}
\label{ne_Eq}
    H(x^{(i)} | \{\hat{y}^{(i)}_j\}_{j=1}^m) = \frac{\sum_{a=1}^{n} \tilde{p}(\hat{y}^{(i)}_a) \log (\tilde{p}(\hat{y}^{(i)}_a))}{\log m}
\end{equation}
where $x^{(i)}$ is the i-th instance of the prompt dataset, m is the number of sampled responses, n is the number of non-repeated responses, $\hat{y}^{(i)}_j$ is the j-th sampled response, and $\hat{y}^{(i)}_{a}$ is the $a$-th non-repeated sampled response.

\begin{table*}[t]
% \captionsetup{font=small}
\caption{Main Results for TriviaQA.} % title
\label{main-results-trivia}
% \resizebox{\textwidth}{!}{%
\small
\centering

\begin{subtable}{\textwidth}
%\caption{}
% First Table
\centering
\scalebox{0.9}{%
%\caption{Results for TriviaQA}
\begin{tabular}{cccccccccccc} % four columns
\toprule[1pt] % change the first line to \toprule
%\multirow{3}{*}{Dataset} & 
\multirow{3}{*}{Methods} & \multirow{3}{*}{\shortstack{Black-Box Access}} & \multicolumn{9}{c}{Error Rate} \\
%\cline{4-12}
%& 
& &\multicolumn{3}{c}{0.2} & \multicolumn{3}{c}{0.25} & \multicolumn{3}{c}{0.3} \\
%& 
& & ECR & SSC$\uparrow$ & APSS$\downarrow$ & ECR & SSC$\uparrow$ & APSS$\downarrow$ & ECR & SSC$\uparrow$ & APSS$\downarrow$ \\
\midrule % change the second line to midrule
%\multirow{6}{*}{TriviaQA}  & 
First-K$_{\text{white}}$ & \ding{55}& 82.1 & 76.6 & 3.39 & 76.1 & 72.9 & 1.90 & \ding{55} & \ding{55} & \ding{55} \\
%& 
CLM & \ding{55}  & 80.2 & 73.4 & 2.29 & 75.2 & 69.1 & 1.55 & 70.1 & 68.3 & 1.28\\
%& 
SCP& \ding{55}  & 80.3 & 75.7 & 2.25 & 75.1 & 70.0 & 1.59 & 70.3 & 74.5 & 1.21\\
%& 
SAPS & \ding{55}  & 80.0 & 77.9 & 2.74 & 75.1 & 64.2 & 1.80 & 70.0 & 49.4 & 1.55\\
%& 
First-K$_{\text{black}}$& {\ding{51}}  & 80.1 & 76.8 & 2.70 & 76.4 & 72.2 & 1.90 & \ding{55} & \ding{55} & \ding{55}\\
%& 
\textbf{BBCP (Ours)} &{\ding{51}}& 80.1 & \textbf{79.0} & \textbf{2.19} & 75.3 & \textbf{74.5} & \textbf{1.43} & 70.3 & \textbf{76.7} & \textbf{1.08}\\
%\bottomrule[1pt] 
\end{tabular}
}
%\vspace{5pt} % Some vertical space between tables

% Second Table
\scalebox{0.9}{%
\begin{tabular}{cccccccccccc} % four columns
\toprule[0.65pt] % change the first line to \toprule
%\multirow{3}{*}{Dataset} & 
\multirow{3}{*}{Methods} & \multirow{3}{*}{\shortstack{Black-Box Access}} & \multicolumn{9}{c}{Error Rate} \\
%\cline{4-12}
%& 
& &\multicolumn{3}{c}{0.35} & \multicolumn{3}{c}{0.4} & \multicolumn{3}{c}{0.45} \\
%& 
& & ECR & SSC$\uparrow$ & APSS$\downarrow$ & ECR & SSC$\uparrow$ & APSS$\downarrow$ & ECR & SSC$\uparrow$ & APSS$\downarrow$ \\
\midrule % change the second line to midrule
%\multirow{6}{*}{TriviaQA}  & 
First-K$_{\text{white}}$ & \ding{55}& \ding{55} & \ding{55} & \ding{55} & 62.4 & 62.5 & 1.00 & \ding{55} & \ding{55} & \ding{55} \\
%& 
CLM & \ding{55}  & 65.0 & 69.3 & 0.96 & 60.1 & 72.7 & 0.81 & 55.2 & 83.3 & 0.70\\
%& 
SCP& \ding{55}  & 65.1 & 76.4 & 1.02 & 60.3 & 75.7 & 0.85 & 55.3 & 82.5 & 0.74\\
%& 
SAPS& \ding{55}  & 65.1 & 57.4 & 1.28 & 60.1 & 70.7 & 0.85 & 55.1 & 76.5 & 0.72\\
%& 
First-K$_{\text{black}}$& {\ding{51}}  & 66.5 & 66.5 & 1.00 & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}\\
%& 
\textbf{BBCP (Ours)} &{\ding{51}}& 65.1 & \textbf{78.5} & \textbf{0.90} & 60.0 & \textbf{81.0} & \textbf{0.75} & 55.2 & \textbf{84.1} & \textbf{0.66}\\
\bottomrule[1pt] % 三线表的粗度
\end{tabular}
}
\vspace{10pt} % Some vertical space between tables
\end{subtable}
\end{table*}

\subsection{Method}

Based on motivations, our nonconformity measures consist of three uncertainty notions: \textit{frequency}, representing the coarse-grained uncertainty; \textit{normalized entropy}, representing the prompt-wise fine-grained uncertainty; and \textit{semantic similarity}, representing the response-wise fine-grained uncertainty. Then we propose the \textbf{B}lack-\textbf{B}ox \textbf{C}onformal \textbf{P}rediction (\textbf{BBCP}) method, which involves three stages: calibration, validation, and testing. Method \ref{LICP} shows the detailed steps. We have also theoretically proven in Appendix \ref{sec:appendix} that our method guarantees marginal coverage.

To be specific, the calibration stage is to find the quantile based on the desired error rate. We sample $m$ responses for each prompt from the LLM $f_{\theta}$, and store them in a response pool constructed in a dictionary structure, where the key is the response, and the value is the frequency that the response occurs. Then we obtain the nonconformity scores of the true label. If the true label exists in the pool, we use the frequency, normalized entropy, and semantic similarity combined nonconformity measures in step \ref{step8} in Method \ref{LICP}; Otherwise, we set the nonconformity score as $\infty$ to signify it is nearly impossible to get the response with true label. Here we define a hyperparameter configuration $\lambda = (\lambda_1, \lambda_2)$, where different values of $\lambda_1$ and $\lambda_2$ are used. Then we find the quantile as the threshold for the later validation stage and test stage. Furthermore, the validation and test stages share the common procedure. The difference is that the validation stage is to choose the best hyperparameter configuration of $\lambda = (\lambda_1, \lambda_2)$, while the test stage is to assess the performance of our method using the configuration selected from the validation. The two stages follow the same sampling procedures as the calibration, then traverse all responses and calculate the frequency, normalized entropy, and semantic similarity combined nonconformity scores. We append the responses whose nonconformity score is less than the quantile score obtained from the calibration stage to our final prediction set.




